Designing a Symbolic Intermediate Representation for Neural Surface Realization

Generated output from neural NLG systems often contain errors such as hallucination, repetition or contradiction. This work focuses on designing a symbolic intermediate representation to be used in multi-stage neural generation with the intention of reducing the frequency of failed outputs. We show that surface realization from this intermediate representation is of high quality and when the full system is applied to the E2E dataset it outperforms the winner of the E2E challenge. Furthermore, by breaking out the surface realization step from typically end-to-end neural systems, we also provide a framework for non-neural content selection and planning systems to potentially take advantage of semi-supervised pretraining of neural surface realization models.

==> failed_sents2.tex <==
%%%%
%KOEL
\begin{table*}[h]
\renewcommand{\arraystretch}{1.6}
\toprule

\begin{subtable}{0.75\textwidth}
\begin{tabular}{rp{27em}}
Generation(I): & priced \textunderscore( it moderately has \textunderscore( but reviews \textunderscore( poor kids \textunderscore( and not )\textunderscore )\textunderscore )\textunderscore )\textunderscore \\[-1ex]
Unusual phrasing(I): &  \\[-1ex]
Nonsensical(I): & shop \textunderscore( xname english rating low english coffee located \textunderscore( xnear centre city )\textunderscore )\textunderscore \\

\end{tabular}
\end{subtable}

\vspace{0.2cm}
\midrule

\begin{subtable}{0.75\textwidth}
\begin{tabular}{rp{27em}}
Generation(G) : & It is moderately priced but has poor reviews and not kids. \\[-1ex]
Unusual phrasing(G): & \\[-1ex]
Nonsensical(G): & Clowns is an English, low rating English coffee shop located near Clare Hall in the city centre. \\
\end{tabular}
\end{subtable}

\vspace{0.2cm}
\midrule

\begin{subtable}{0.75\textwidth}
\begin{tabular}{rp{27em}}
Generation(R): & It is moderately priced but has poor reviews, and not for kids.\\[-1ex]
Unusual phrasing(R): &   \\[-1ex]
Nonsensical(R): & The Clowns is a english low rating english coffee shop located near Clare Hall in the city centre.  \\
\end{tabular}
\end{subtable}

\vspace{.2cm}

\bottomrule
\vspace{0.3cm}
\caption{Examples of reference sentences, intermediate representations and generated texts from three difference scenarios, i.e,... G: the generated input. I: the intermediate representations. R: the reference.  }\label{tab:results:examples}
\end{table*}
%%%%%
